Integration of a machine learning model into a decision support tool to predict absenteeism at work of prospective employees

Purpose - Inefficient hiring may result in lower productivity and higher training costs. Productivity losses caused by absenteeism at work cost U.S. employers billions of dollars each year. Also, employers typically spend a considerable amount of time managing employees who perform poorly. The purpose of this study is to develop a decision support tool to predict absenteeism among potential employees. Design/methodology/approach - We utilized a popular open-access dataset. In order to categorize absenteeism classes, the data have been preprocessed, and four methods of machine learning classification have been applied: Multinomial Logistic Regression (MLR), Support Vector Machines (SVM), Artificial Neural Networks (ANN), and Random Forests (RF). We selected the best model, based on several validation scores, and compared its performance against the existing model; we then integrated the best model into our proposed web-based for hiring managers. Findings - A web-based decision tool allows hiring managers to make more informed decisions before hiring a potential employee, thus reducing time, financial loss and reducing the probability of economic insolvency. Originality/value - In this paper, we propose a model that is trained based on attributes that can be collected during the hiring process. Furthermore, hiring managers may lack experience in machine learning or do not have the time to spend developing machine learning algorithms. Thus, we propose a web-based interactive tool that can be used without prior knowledge of machine learning algorithms.

==> references.tex <==


\begin{thebibliography}{}
	
	
	\bibitem[Abiodun \textit{et~al}(2018)]{Abiodun_2018}
	Abiodun, O.~I., Jantan, A., Omolara, A.~E., Dada, K.~V., Mohamed, N.~A. and Arshad, H. (2018), ``State-of-the-art in artificial neural network applications: A survey'',  \emph{Heliyon}, Vol.4 No.11, e00938. https://doi.org/10.1016/j.heliyon.2018.e00938
	
	
	
	\bibitem[Agrestik(2002)]{Agresti_2002}
	Agresti, A. (2002), \emph{Categorical data analysis}, John Wiley \& Sons, Hoboken, NJ. https://doi.org/10.
1198/tech.2003.s28
	
	
	
	
	\bibitem[Bradley(1997)]{Bradley_1997}
	Bradley, A.~P.  (1997), ``The use of the area under the ROC curve in the
	evaluation of machine learning algorithms'',  \emph{Pattern Recognition}, Vol. 30 No. 7, pp. 1145-1159. https://doi.org/10.1016/S0031-3203(96)00142-2
	
	
	
	
	\bibitem[Cervantes \textit{et~al.}(2020)]{Cervantes_2020}
	Cervantes, J., Lamont, G.~ F.,  Mazahua, R.~M.~A.~L.  and Lopez A. (2020), ``A comprehensive survey on support vector machine classification: Applications, challenges and trends,
	Neurocomputing'',  \emph{Neurocomputing}, Vol. 408, pp. 189-215. https://doi.org/10.1016/j.neucom.2019.10.118
	
	
	
	
	\bibitem[Delen \textit{et~al.}(2007)]{Delen_2007}
	Delen, D., Sharda, R. and Kumar, P. (2007),  ``Movie forecast guru: A web-based DSS for hollywood managers'',  \emph{Decision Support Systems}, Vol. 43~No. 4, pp. 1151-1170. https://doi.org/10.1016/j.dss.2005.07.005
	
	
	
	\bibitem[Fawcett(2006)]{Fawcett_2006}
	Fawcett, T. (2006), ``An introduction to ROC analysis'', \emph{Pattern Recognition Letters}, Vol. 27, pp. 861-874. https://doi.org/10.1016/j.patrec.2005.10.010
	
	
%	\bibitem[Ferreira et~al.(2018)Ferreira, Martiniano, Napolitano, Farias \& Sassi]{Ferreira_2018}
%	Ferreira, R.~P., Martiniano, A., Napolitano, D., Farias, E.~B.~P., \& Sassi, R.~J. (2018). Artificial Neural Network and their Application In the Prediction of Absenteeism at Work. \emph{International Journal of Recent Scientific Research}, \emph{9}(1), 23332--23334.
	
	
	% Double check if there is any DOI or can we change this refference? 
	\bibitem[Gayathri(2005)]{Gayathri_2018}
	Gayathri, T. (2018), ``Data mining of absentee data to increase productivity'', \emph{International Journal of engineering and techniques}, Vol. 4 No. 3, pp. 478-480. http://www.ijetjournal.org/Volume4/Issue3/IJET-V4I3P78.pdf
	
	
	
		\bibitem[Hallinan(2013)]{Hallinan_2013}
	Hallinan, S.~J. (2013), ``Computational Intelligence in the Design of Synthetic Microbial Genetic Systems'',  
 Harwood, 	C.  and    Wipat, A. (Eds.), \emph{Methods in Microbiology}, Vol. 40,  Elsevier, pp.  1-37.  https://doi.org/10.1016/B978-0-12-417029-2.00001-7
	
	
	
	\bibitem[Halpern \textit{et~al.}(2001)]{Halpern_2001}
	Halpern, M.~T., Shikiar, R., Rentz A.~M. and  Khan,  Z. M. (2001), ``Impact of smoking status on workplace absenteeism and productivity'', \emph{Tobacco control}, Vol. 10 No.3,  pp. 233-238. http://dx.doi.org/10.1136/tc.10.3.233
	
	

	
	\bibitem[Hanley and  McNeil(1982)]{Hanley_1982}
	Hanley, J.~A.  and  McNeil, B. J.      (1982), ``The meaning and use of the
	area under a receiver operating characteristic (ROC) curve'',  \emph{Radiology},  Vol. 143, pp. 29--36.  http://dx.doi.org/10.1148/radiology.143.1.7063747 
	


\bibitem[Imran \textit{et~al.}(2019)]{Imran_2019}
Imran, A.~A.,  Amin, M.~N.,  Rifat, M.~R. and  Mehreen, S.  (2019),  ``Deep Neural Network Approach for predicting the productivity of garment employees'', \emph{IEEE, 6th International Conference on Control, Decision and Information Technologies (CoDIT)}, pp. 1402-1407. http://dx.doi.org/10.1109/CoDIT.2019.8820486


\bibitem[Johnson and  Khoshgoftaar(2019)]{Johnson_2019}
Johnson, J.M. and   Khoshgoftaar, T.M. (2019), ``Survey on deep learning with class imbalance'',  \emph{Journal of Big Data},  Vol. 6 No. 27. https://doi.org/10.1186/s40537-019-0192-5





\bibitem[Kim, Hong  and Park(2018)]{Kim_2018}
Kim, J.,  Hong, J.  and Park, H (2018), ``Prospects of deep learning for medical imaging'', \emph{Precision and Future Medicine},  Vol. 2 No. 2, pp. 37-52. https://doi.org/10.23838/pfm.2018.00030


	
	
	\bibitem[Kocakulah \textit{et~al.}(2016)]{Kocakulah_2016}
	Kocakulah, M.~C., Kelley, A.~G., Mitchell, K.~M. and Ruggieri, M.~P. (2016), ``Absenteeism problems and costs: causes, effects and cures'', \emph{International Business \& Economics Research Journal (IBER)}, Vol. 15 No. 3, pp. 89-96. https://doi.org/10.19030/iber.v15i3.9673
	
	
	
	
	\bibitem[Kulkarni \textit{et~al.}(2020)]{Kulkarni_2020}
	Kulkarni, A., Chong, D. and  Batarseh, F.~A. (2020),  ``Foundations of data imbalance and solutions for a data democracy'', Batarseh, F. A.  and   Yang, R.
	(Eds.), \emph{Data Democracy},  Academic Press, pp.  83-106. https://doi.org/10.1016/B978-0-12-818366-3.00005-8
	

	
	
	\bibitem[Leonard(2017)]{Leonard_2017}
	Leonard, L.~C. (2017), ``Web-based behavioral modeling for continuous user authentication (CUA)'',  Memon, A.~M. (Ed.),  Vol. 105, Elsevier,  pp.  1-144. https://doi.org/10.1016/bs.adcom.2016.12.001
	
	
	
	\bibitem[Luque \textit{et~al.}(2019)]{Luque_2019}
	Luque, A.,  Carrasco,A., Martin, A. and  Heras, A. (2019), ``The impact of class imbalance in classification performance metrics based on the binary confusion matrix'',  \emph{Pattern Recognition}, Vol. 91, pp. 216-231. https://doi.org/10.1016/j.patcog.2019.02.023
	
	
	
	
	\bibitem[Martiniano \textit{et~al.}(2012)]{Martiniano_2012}
	Martiniano, A., Ferreira, R.~P., Sassi, R.~J. and Affonso, C. (2012), ``Application of a neuro fuzzy network in prediction of
	absenteeism at work'',  \emph{In Information Systems and
		Technologies, 7th Iberian Conference}, pp. 1-4. https://ieeexplore.ieee.org/document/6263151
	
	
	
	
	\bibitem[Navarro and  Bass(2006)]{Navarro_2006}
	Navarro, C. and  Bass, C. (2016), ``The Cost of Employee Absenteeism'',  \emph{Sage journals}, Vol. 38 No. 6, pp. 26-30. https://doi.org/10.1177/0886368706295343
	
	
	%did not find https
%	\bibitem[Neuborne(2003)]{Neuborne_2003}
%	Neuborne, E. (2003). The carrot, not the stick. \emph{Potentials}, \emph{36}, 39--41.
	



\bibitem[Saarela  and  Jauhiainen(2021)]{Saarela_2021}
Saarela, M. and  Jauhiainen, S. (2021), ``Comparison of feature importance measures as explanations for classification models'',   \emph{SN Applied Sciences},  Vol. 3 No. 272. https://doi.org/10.1007/s42452-021-04148-9



\bibitem[Sarica  \textit{et~al.}(2017)]{Sarica_2017}
Sarica A, Cerasa A, and  Quattrone, A. (2017). ``Random forest algorithm for the classification of neuroimaging data in Alzheimer's disease: A systematic review''.  \emph{Front. Aging Neurosci.}, Vol. 9 No. 329.  https://doi.org/10.3389/fnagi.2017.00329



\bibitem[Shah  \textit{et~al.}(2020)]{Shah_2020}
Shah, S.~A. ~A., Uddin, I., Aziz, F., Ahmad, S., Al-Khasawneh, M.~A. and  Sharaf,  M. (2020), ``An enhanced deep neural network for predicting workplace absenteeism'',  \emph{Complexity}, Vol. 2020 No. 5843932. https://doi.org/10.1155/2020/5843932




\bibitem[Simsek  \textit{et~al.}(2021)]{Simsek_2021}
Simsek, S., Albizri, A., Johnson, M., Custis, T. and  Weikert, S. (2021), ``Predictive data analytics for contract renewals: a decision support tool for  managerial decision-making'',  \emph{Journal of Enterprise Information Management},  Vol. 34 No. 2, pp.  718-732. https://doi.org/10.1108/JEIM-12-2019-0375



\bibitem[Simsek \textit{et~al.}(2020)]{Simsek_2020}
Simsek, S.,   Genc, O.,   Albizri, A.,  Dinc, S. and   Gonen, B. (2020), ``Artificial neural network incorporated decision support tool for point velocity prediction'',  \emph{Journal of Business Analytics}, Vol. 3 No.1, pp. 67-78. https://doi.org/10.1080/2573234X.2020.1751569





\bibitem[Simpson(2011)]{Simpson_2011}
Simpson, I. (2011),  ``Ailing and overweight Americans cost billions in productivity'', \emph{Reuters}, 17 October.    Retrieved from https://www.reuters.com/article/us-absenteeism-idUSTRE79G17X20111017



\bibitem[Skorikov \textit{et~al.}(2020)]{Skorikov_2020}
Skorikov, M., Hussain, M. R., Akbar, M. K., Momen, S., Mohammed, N. and  Nashin, T.  (2020), ``Prediction of absenteeism at work using data mining techniques'',  \emph{IEEE, 5th International Conference on Information Technology Research}, pp.  1-6. https://doi.org/10.1109/ICITR51448.2020.9310913



\bibitem[Suthaharan S.(2016)]{Suthaharan_2016}
Suthaharan, S.   (2016), ``A cognitive random forest: an intra- and intercognitive computing for big data classification under cune condition'', Gudivada, V.~N.,   Raghavan,V.~V.,   Govindaraju, V. and  Rao, C.~R.  (Eds.), \emph{Handbook of Statistics},  Vol. 35,  Elsevier,  pp. 207-227.  https://doi.org/10.1016/bs.host.2016.07.006 
%In V.~N. Gudivada, V.~V. Raghavan, V. Govindaraju, \&  C.~R. Rao, (Eds.)


\bibitem[Sun  \textit{et~al.}(2020)]{Sun_2020}
Sun, J., Li, H., Fujita, H., Fu, B. and Ai, W. (2020), ``Class-imbalanced
dynamic financial distress prediction based on adaboost-SVM
ensemble combined with SMOTE and time weighting'', \emph{Information Fusion},  Vol. 54, pp. 128-144. https://doi.org/10.1016/j.inffus.2019.07.006


\bibitem[Tunceli  \textit{et~al.}(2005)]{Tunceli_2005}
Tunceli, K., Bradley, C. J., Nerenz, D., Williams,  L. K., Pladevall,  M. and  Lafata, J. E.   (2005),  ``The impact of diabetes on employment and work productivity'',  \emph{Diabetes Care}, Vol. 28 No. 11, pp. 2662-2667.  https://doi.org/10.2337/diacare.28.11.2662


\bibitem[Vapnik(1998)]{Vapnik_1998}
Vapnik, V.~N (2002), ``Consistency of Learning Processes'', \emph{The Nature of Statistical Learning Theory}, Springer, New York, NY.    https://doi.org/10.1007/978-1-4757-3264-1\_3



\bibitem[Yadav \textit{et~al.}(2018)]{Yadav_2018}
Yadav, A.~ M.,  Chaurasia, R.~C.,  Suresh, N. and Gajbhiye, P. (2018), ``Application of artificial neural networks and response surface methodology approaches for the prediction of oil agglomeration process'',  \emph{Fuel}, Vol. 220, pp. 826-836. https://doi.org/10.1016/j.fuel.2018.02.040


\bibitem[Young \textit{et~al.}(2014)]{Young_2014}
Young II, W. A., Bihl, T. J. and  Weckman, G. R. (2014), ``Artificial Neural Networks for Business Analytics'',  Wang, J. (Ed.),  \textit{Encyclopedia of Business Analytics and Optimization}, Vol. 40, IGI Global,  Hershey, PA, pp.193-208. https://doi.org/10.4018/978-1-4666-5202-6.ch019



\bibitem[Zhang  and  Dou(2021)]{Zhang_2021}
Zhang, K., Su, H. and  Dou, Y.  (2021), ``Beyond AP: a new evaluation index for multiclass classification task accuracy'',   \emph{Applied Intelligence}, Vol. 51, pp. 7166–7176. https://doi.org/10.1007/s10489-021-02223-7



\end{thebibliography}

